Verifying Unboundedness via Amalgamation

Well-structured transition systems (WSTS) are an abstract family of systems that encompasses a vast landscape of infinite-state systems. By requiring a well-quasi-ordering (wqo) on the set of states, a WSTS enables generic algorithms for classic verification tasks such as coverability and termination. However, even for systems that are WSTS like vector addition systems (VAS), the framework is notoriously ill-equipped to analyse reachability (as opposed to coverability). Moreover, some important types of infinite-state systems fall out of WSTS' scope entirely, such as pushdown systems (PDS). Inspired by recent algorithmic techniques on VAS, we propose an abstract notion of systems where the set of runs is equipped with a wqo and supports amalgamation of runs. We show that it subsumes a large class of infinite-state systems, including (reachability languages of) VAS and PDS, and even all systems from the abstract framework of valence systems, except for those already known to be Turing-complete. Moreover, this abstract setting enables simple and general algorithmic solutions to unboundedness problems, which have received much attention in recent years. We present algorithms for the (i) simultaneous unboundedness problem (which implies computability of downward closures and decidability of separability by piecewise testable languages), (ii) computing priority downward closures, (iii) deciding whether a language is bounded, meaning included in $w_1^*\cdots w_k^*$ for some words $w_1,\ldots,w_k$, and (iv) effective regularity of unary languages. This leads to either drastically simpler proofs or new decidability results for a rich variety of systems.

==> Configuration/fonts.tex <==
%
\setmainfont[Ligatures=TeX]{Liberation Serif}
\setmonofont[
	Path = {./Fonts/SourceCodePro/},
	Ligatures = TeX,
	Extension = .otf,
	UprightFont = *-Regular,
	ItalicFont = *-It,
	BoldFont = *-Bold,
	BoldItalicFont = *-BoldIt,
    Scale = MatchLowercase,
    Scale = 0.95
]{SourceCodePro}



==> Configuration/knowledge.tex <==
%
\knowledge{notion}
| alphabet
\knowledge{notion}
| subword
\knowledge{notion}
| downward closure
\knowledge{notion}
| tree
| trees
\knowledge{notion}
| subtree
\knowledge{notion}
| Simultaneous Unboundedness
| Simultaneous Unboundedness Problem
| SUP
\knowledge{notion}
| run embedding
\knowledge{notion}
| amalgamation
| amalgamations
| amalgamation system
| system with amalgamations
\knowledge{notion}
| effective@amlgm
\knowledge{notion}
| pumpable embedding
| pumpable embeddings
\knowledge{notion}
| PVASS
| pushdown vector addition system with states
| pushdown vector addition system
\knowledge{notion}
| configuration@PVASS
\knowledge{notion}
| run@PVASS
| runs@PVASS
\knowledge{notion}
| VASS grammar
| VASS grammars
\knowledge{notion}
| terminal@VASSG
\knowledge{notion}
| accepting@VASSG
\knowledge{notion}
| valid@VASSG
\knowledge{notion}
| derivation tree
| derivation trees
| tree@VASSG
\knowledge{notion}
| initial counter value
\knowledge{notion}
| final counter value
\knowledge{notion}
| action
| actions
| action@VASSG
\knowledge{notion}
| lifting
| liftings
\knowledge{notion}
| inhibitor
| inhibitors
| zero-test
| zero-tests
\knowledge{notion}
| hierarchical inhibitor
| hierarchical inhibitors
| nested zero-test
| nested zero-tests
\knowledge{notion}
| HI-PVASS


\let\subwordplain\subword
\renewcommand\subword{\mathrel{\kl[\subword]\subwordplain}}

\newcommand\dc[1]{#1{\kl[\dc]\downarrow}}

\newcommand\vleq{\mathrel{\kl[\vleq]\leq}}
\newcommand\vlt{\mathrel{\kl[\vlt]{<}}}
\newcommand\vstrictlt{\mathrel{\kl[\vstrictlt]\ll}}
\newcommand\prefixleq{\mathrel{\kl[\prefixleq]{\leq_p}}}
\newcommand\prefixnleq{\mathrel{\kl[\prefixleq]{\not{\leq_p}}}}

\newcommand\Trees[1]{\kl[\Trees]{{T}}(#1)}
\newcommand\leaf[1]{#1\kl[\leaf]{[]}}
\newcommand\tree[2]{#1{\kl[\tree]{[}#2\kl[\tree]{]}}}
\newcommand\subtree[2]{#1\kl[\subtree]{/}#2}

\let\rootnodeplain\rootnode
\renewcommand\rootnode[1]{\kl[\rootnode]{\rootnodeplain}(#1)}


\let\runembedplain\runembed
\renewcommand\runembed{\mathrel{\kl[\runembed]\runembedplain}}
\newcommand\liftembed[1]{\mathrel{\kl[\liftembed]{\runembedplain}^{#1}}}


\let\yieldplain\yield
\renewcommand\yield[1]{\kl[\yield]\yieldplain(#1)}

\newcommand\gap[2]{\kl[\gap]{gap_{#1}^{#2}}}

\newcommand\pvQ{\kl[\pvQ]{Q}}
\newcommand\pvAlph{\kl[\pvAlph]\Sigma}
\newcommand\pvStck{\kl[\pvStck]\Gamma}
\newcommand\pvT{\kl[\pvT]{T}}
\newcommand\pvInit{\kl[\pvInit]{q_0}}
\newcommand\pvFinal{\kl[\pvFinal]{F}}
\newcommand\pvAct{\kl[\pvAct]{Act_n}}
\newcommand\vgN{\kl[\vgN]{N}}
\newcommand\vgAlph{\kl[\vgAlph]{\Sigma}}
\newcommand\vgP{\kl[\vgP]{P}}
\newcommand\vgS{\kl[\vgS]{S}}

\newcommand\vassQ{\kl[\vassQ]{Q}}
\newcommand\vassInit{\kl[\vassInit]{q_0}}
\newcommand\vassT{\kl[\vassT]{T}}
\newcommand\vassF{\kl[\vassF]{q_f}}
\newcommand\vassAct{\kl[\vassAct]{Act_n}}
\newcommand\vassAlph{\kl[\vassAlph]\Sigma}
\newcommand\vassC{\kl[\vassC]{C}}
\newcommand\vassSteps{\kl[\vassSteps]{Steps}}

\newcommand\vFirst{\kl[\vFirst]{\mathrm{first}}}
\newcommand\vLast{\kl[\vLast]{\mathrm{last}}}

\newcommand\treesubst[3]{#1\kl[\treesubst]{[}#2 \mathrel{\kl[\treesubst]\mapsto} #3\kl[\treesubst]{]}}

\newcommand\vassLiftEmbed[2][]{\mathrel{\kl[\vassLiftEmbed]\runembedplain^{#2}_{#1}}}

\newcommand\supexp[1]{\kl[\supexp]\eta(#1)}


